A Study of Checkpointing in Large Scale Training of Deep Neural Networks

Deep learning (DL) applications are increasingly being deployed on HPC systems, to leverage the massive parallelism and computing power of those systems for DL model training. While significant effort has been put to facilitate distributed training by DL frameworks, fault tolerance has been largely ignored. In this work, we evaluate checkpoint-restart, a common fault tolerance technique in HPC workloads. We perform experiments with three state-of-the-art DL frameworks common in HPC Chainer, PyTorch, and TensorFlow). We evaluate the computational cost of checkpointing, file formats and file sizes, the impact of scale, and deterministic checkpointing. Our evaluation shows some critical differences in checkpoint mechanisms and exposes several bottlenecks in existing checkpointing implementations. We provide discussion points that can aid users in selecting a fault-tolerant framework to use in HPC. We also provide takeaway points that framework developers can use to facilitate better checkpointing of DL workloads in HPC.

==> authors.tex <==


% \author{\IEEEauthorblockN{Author 1}
% \IEEEauthorblockA{\textit{National University of Costa Rica} \\
% \textit{School of Computing,}\\
% \textit{Institution 2}\\
% San Jos\'e, Costa Rica \\
% email}
% \and
% \IEEEauthorblockN{Author 2}
% \IEEEauthorblockA{\textit{ }\\\textit{Institution 2}\\
% San Jos\'e, Costa Rica \\
% email}

% \and
% \IEEEauthorblockN{Author 3}
% \IEEEauthorblockA{\textit{Institution 1 }\\\textit{Institution 2}\\
% San Jos\'e, Costa Rica \\
% email}

% \and
% \IEEEauthorblockN{Author 4}
% \IEEEauthorblockA{\textit{Institution 1 %}\\\textit{Institution 2}\\
% San Jos\'e, Costa Rica \\
% email}
% }

\author{Elvis Rojas\affilnum{1,3}, Albert Njoroge Kahira\affilnum{4,5}, Esteban Meneses\affilnum{2,3}, Leonardo Bautista Gomez\affilnum{4} and Rosa M Badia\affilnum{4,5}}

\affiliation{\affilnum{1}National University of Costa Rica, Costa Rica\\
\affilnum{2}Costa Rica National High Technology Center, Costa Rica\\
\affilnum{3}Costa Rica Institute of Technology, Costa Rica \\
\affilnum{5},Universitat Politècnica de Catalunya \\
\affilnum{4}Barcelona Supercomputing Center, Spain \\
\affilnum{5}Universitat Politècnica de Catalunya, Spain
}

\corrauth{Elvis Rojas, National University of Costa Rica, Costa Rica}

\email{erojas@una.ac.cr}



==> old/old_discussion.tex <==

\section{Discussion}\label{sec:discussion}

In this section, we present key findings and discussion points that emerged from this study. First, we emphasize that checkpointing is an integral part of Deep Learning workloads in HPC. Our study has exposed several insights that can help both framework developers and framework users when training DL models in HPC. 

\begin{itemize}
    \item \textbf{\emph{Impact of Scale: }} Increasing the number of GPUs during training significantly improves the training time of DL models. However, it has no impact on the checkpointing time as checkpointing is done by only one GPU. Though Chainer has some sort of multi GPU implementation, our study showed that this simply produces redundant copies of the checkpoint and does not improve the time to checkpoint. There is therefore an opportunity for external libraries typically used in HPC for checkpointing in DL workloads. However such frameworks would have to be heavily modified to facilitate checkpointing in data parallelism. The challenge in this is that in data parallelism all process have a replica of the model and all perform an all reduce operation at the end of an iteration. One possible solution would be to shard the model such that each process checkpoints a small part of the model. There is already some promising work done along this line by \cite{! }. However the work is not conclusive since no analysis was performed on the cost of  reconstructing the model and restarting. 
    
   
    \item \textbf{\emph{Data parallel vs model parallel: checkpoint strategies, pros and cons.}} Though this study primarily focused on Data parallelism, its also important to consider model parallelism especially now that model parallelism is becoming common due to increase in model sizes. As mentioned earlier, in data parallelism, there is a replica of the model on each GPU. However, in Model Parallelism, the model is split between process and each process trains a part of the model. This is a challenge to existing checkpointing implementations as they don't do partial checkpoints. 
    
    
    
    
    \item \textbf{\emph{Checkpoint file format}}: diversity, scalability, size, optimization opportunities. We observe that each framework has its own file format for saving checkpoints. This is expected as the checkpoint mechanism is not standard. There are clear differences between the file sizes due to the choice of file formats. For instance, chainer is able to significantly compress checkpoint files depending on the model. To facilitate using existing checkpointing libraries for DL workloads, the file format should be addressed. For instance, a framework agnostic checkpointing library should be able to checkpoint in a single file format but the frameworks should be able to resume from this format.
    
    
    \item \textbf{\emph{Checkpoint implementations:}}
        All existing DL frameworks include  the ability to checkpoint during training in a native way.  However, DL frameworks have evolved to adapt to new HPC systems that allow distributed training without taking checkpoint processes into account.

Currently there are checkpointing libraries specifically designed for HPC applications~\cite{fti,veloc} that are optimized for better performance under distributed processing conditions.  As described in~\cite{nicolae}, there is already an effort to implement in DL applications a checkpoint library developed for HPC environments.  The idea behind is to offer DL applications advanced features such as asynchronous multi-level checkpointing, hiding the complexity of heterogeneous storage, or the efficient serialization on local storage, which are some of the fundamental elements to obtain the maximum performance.

Currently, DL framework developers are probably more interested in optimizing, debugging, and standardizing the mechanisms that drive distributed training.  At some point they will have to turn their gaze to the checkpoint processes that will take on more relevance as training times increase and checkpoint file sizes grow, punishing the scaling.  With this scenario, we can think that the implementation of already developed checkpoint libraries is a good choice to solve the possible drawbacks of checkpointing in DL distributed applications.  However, efforts to carry out this type of implementations so far are few and it is not known if the developers of DL frameworks are interested in taking the ideas from the existing checkpointing libraries and adding them to their frameworks or developing native implementations with the same features needed to take advantage of HPC systems.

 \item \textbf{\emph{Deterministic behavior in DNN: }} Currently the implementation of determinism in DL models is a secondary element. This can be considered normal and desirable because ANNs have a random nature that seeks to model the behavior of neurons in a biological brain.  However, the randomness of the results can raise reasonable doubts about their veracity as they are not reproducible, especially when DL models grow in complexity and are susceptible to failures.  At the end of this work, we realized that the options offered by DL frameworks to generate 100\% deterministic results in training and when restarting a training (deterministic restart) are not entirely reliable to generate the expected result.  In some cases the developers themselves do not ensure complete deterministic behaviors between versions and/or platforms (hardware, software).  It is necessary that DL frameworks provide clear and easy-to-implement mechanisms that allow the reproducibility of results and therefore research environments that allow validation of the experiments.

    
\end{itemize}






